Training of SSD(Single Shot Detector) for Facial Detection using Nvidia Jetson Nano

In this project, we have used the computer vision algorithm SSD (Single Shot detector) computer vision algorithm and trained this algorithm from the dataset which consists of 139 Pictures. Images were labeled using Intel CVAT (Computer Vision Annotation Tool) We trained this model for facial detection. We have deployed our trained model and software in the Nvidia Jetson Nano Developer kit. Model code is written in Pytorch's deep learning framework. The programming language used is Python.

==> glossary.tex <==
\newacronym{ucp}{UCP}{University of Central Punjab}

\newacronym{who}{WHO}{(World Health Organization)}
\newacronym{ssd}{SSD}{(Single Shot Detector)}
\newacronym{rcnn}{R-CNN}{(Region-based Convolutional Neural Networks)}
\newacronym{frcnn}{Fast R-CNN}{(Region-based Convolutional Neural)} 
\newacronym{mAP}{mAP}{(mean Average Precision)} 
\newacronym{voc}{VOC}{(Visual Object Classes)} 
\newacronym{coco}{COCO}{(Common Objects in Context)} 
\newacronym{ilsvrc}{ILSVRC}{(ImageNet Large Scale Visual Recognition Challenge)}
